Subspace Hybrid MVDR Beamforming for Augmented Hearing

Signal-dependent beamformers are advantageous over signal-independent beamformers when the acoustic scenario - be it real-world or simulated - is straightforward in terms of the number of sound sources, the ambient sound field and their dynamics. However, in the context of augmented reality audio using head-worn microphone arrays, the acoustic scenarios encountered are often far from straightforward. The design of robust, high-performance, adaptive beamformers for such scenarios is an on-going challenge. This is due to the violation of the typically required assumptions on the noise field caused by, for example, rapid variations resulting from complex acoustic environments, and/or rotations of the listener's head. This work proposes a multi-channel speech enhancement algorithm which utilises the adaptability of signal-dependent beamformers while still benefiting from the computational efficiency and robust performance of signal-independent super-directive beamformers. The algorithm has two stages. (i) The first stage is a hybrid beamformer based on a dictionary of weights corresponding to a set of noise field models. (ii) The second stage is a wide-band subspace post-filter to remove any artifacts resulting from (i). The algorithm is evaluated using both real-world recordings and simulations of a cocktail-party scenario. Noise suppression, intelligibility and speech quality results show a significant performance improvement by the proposed algorithm compared to the baseline super-directive beamformer. A data-driven implementation of the noise field dictionary is shown to provide more noise suppression, and similar speech intelligibility and quality, compared to a parametric dictionary.

==> _acknowledgement.tex <==
\section*{Acknowledgement}
\label{sec:acknowledgement}
The authors would like to thank the associated editor and the reviewers for their constructive comments and suggestions, which have significantly benefited the paper.

==> _introduction_backup.tex <==
\section{Introduction}
\label{sec:introduction2}
% \acresetall

Colin Cherry was the first to identify the `cocktail party problem' as the task of enhancing one target signal, or voice, in the presence of multiple interfering signals and noise \citep{Cherry1953,Bronkhorst2000}. Despite advances in speech enhancement and microphone array processing, the cocktail party problem still remains a challenge in the audio signal processing community after decades of research \citep{Bronkhorst2000,Donley2021a,SPEARwebsite}. Relevant applications include teleconferencing, speech recognition in human-machine interactions, hearing aids, and augmented reality audio. 

It is widely known that significant enhancement can be achieved using the acoustic signals captured with a microphone array device \citep{Doclo2010,Lollmann2017,Klasen2007,HaebUmbach2019}. The use of wearable microphone arrays is a beguiling approach towards addressing the cocktail party problem. Wearable arrays, such as \ac{AR} glasses \citep{Donley2021a}, can additionally provide head/array position and orientation information, as well as source \acp{DOA} and/or other environmental information obtained using a camera or other sensors. However, the compact size and real-world implementation of such systems restricts the processing to be computationally inexpensive, causal, real-time and robust to unforeseen scenarios. This paper addresses scenarios with one or more target talkers in the presence of localized interferers and ambient noise, using a head-worn microphone array mounted in \ac{AR} glasses. It is assumed in the following that the array's \acp{ATF} and the target \acp{DOA} are known with realistic accuracy.

Multichannel speech enhancement systems \citep{Benesty2008b} typically employ \ac{MISO} algorithms exploiting spatial, temporal and spectral information to improve the \ac{SNR} at the output. The potential for additional improvement using \ac{SISO} post-processing, such as the Wiener filter \citep{Wiener1949}, spectral subtraction \citep{Loizou2007} or \ac{DL}-based methods \citep{Hu2020a,Luo2018a} is recognized but not studied here; the focus in this work is the \ac{MISO} block in such systems. Without loss of generality, a multi-target scenario is considered as multiple single-target scenarios in which the same \ac{MISO} method can be applied. Such decomposition of the scenario is known to improve the enhancement performance due to the use of fewer distortionless target constraints and correspondingly increase the potential for noise suppression. In addition, it enables control of the mixture of enhanced sources in the output depending on the application.

In this work, a novel analytical beamforming algorithm is proposed which is causal and able to adapt to complex and non-isotropic noise fields while being computationally efficient due to the use of pre-calculated weights. The dictionary of precalculated beamformer weights is shown to have the flexibility of being analytical (parametric) or data-driven. Early work on this topic was described in \citep{Hafezi2023}. Here, the work has been extended to include a new formulation, the data-driven dictionary, more extensive evaluations and mathematical analysis of the method.

The remainder of the paper is structured as follows. Section~\ref{sec:backgroundReview} provides a brief review of beamforming approaches. Section~\ref{sec:problemformulation} formulates the problem and defines the baseline beamformer. Sections~\ref{sec:method} and \ref{sec:dictionary} respectively propose the multichannel enhancement system and two categories of parametric and data-driven dictionaries of beamformer weights. Section~\ref{sec:evaluation} compares the two implementations of the proposed method with the baseline beamformer using real-world recordings and simulated cocktail party data with a head-worn microphone array. Finally, conclusions are given in Section~\ref{sec:conclusion}.


==> appendices.tex <==
% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%
\appendices
\input{minimisation_proof}
\label{sec:minimisation}


% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
% \section{}
% % \input{appendix_two}
% Appendix two text goes here.
% \appendix
% \label{appendix:minimisation_proof}
% \input{minimisation_proof}


==> bibitems.tex <==
\bibitem[\protect\astroncite{Avargel and Cohen}{2007}]{Avargel2007a}
Y.~Avargel and I.~Cohen, ``On multiplicative transfer function approximation in
  the short-time {{Fourier}} transform domain,'' \emph{{IEEE} Signal Process.
  Lett.}, vol.~14, no.~5, pp. 337--340, 2007.

%\bibitem[\protect\astroncite{Avargel and Cohen}{2007}]{Avargel2007a}
%Y.~Avargel and I.~Cohen, ``On multiplicative transfer function approximation in
 % the short-time {{Fourier}} transform domain,'' \emph{{IEEE} Signal Process.
 % Lett.}, vol.~14, no.~5, pp. 337--340, 2007.
  
\bibitem[\protect\astroncite{Bitzer and Simmer}{2001}]{Bitzer2001a}
J.~Bitzer and K.~U. Simmer, ``Superdirective microphone arrays,'' in
  \emph{Microphone {{Arrays}}: {{Signal Processing Techniques}} and
  {{Applications}}}, M.~S. Brandstein and D.~B. Ward, Eds.\hskip 1em plus 0.5em
  minus 0.4em\relax Berlin, Germany: Spring{\-}er-Ver{\-}lag, 2001, pp. 19--38.

\bibitem[\protect\astroncite{Braun and Habets}{2015}]{Braun2015}
S.~Braun and E.~A.~P. Habets, ``A multichannel diffuse power estimator for
  dereverberation in the presence of multiple sources,'' \emph{{EURASIP} J. on
  Audio, Speech, and Music Processing}, vol. 2015, no.~1, p.~34, Dec. 2015.
  
\bibitem[\protect\astroncite{Boersma \textit{et al.}}{2020}]{Boersma2020}
P. Boersma, and D. Weenink, ``Praat: doing phonetics by computer,'' \emph{[computer program]}, Version 6.1.09, retrieved 26 January 2020, http://www.praat.org, 2020.
  
\bibitem[\protect\astroncite{Braun \textit{et al.}}{2018}]{Braun2018a}
S.~Braun, A.~Kuklasi\'nski, O.~Schwartz, O.~Thiergart, E.~A.~P. Habets,
  S.~Gannot, S.~Doclo, and J.~Jensen, ``Evaluation and comparison of late
  reverberation power spectral density estimators,'' \emph{{IEEE/ACM} Trans.
  Audio, Speech, Lang. Process.}, vol.~26, no.~6, pp. 1056--1071, June 2018.

\bibitem[\protect\astroncite{Brookes}{1997}]{Brookes1997}
D.~M. Brookes, ``{{VOICEBOX}}: {{A}} speech processing toolbox for
  {{MATLAB}},'' 1997--2016. [Online]. Available:
  \url{http://www.ee.ic.ac.uk/hp/staff/dmb/voicebox/voicebox.html}
  
\bibitem[\protect\astroncite{Capon \textit{et al.}}{1969}]{Capon1969}
J.~Capon, ``High resolution frequency-wavenumber spectrum analysis,''
  \emph{Proc. {IEEE}}, vol.~57, pp. 1408--1418, Aug. 1969.

\bibitem[\protect\astroncite{Chakrabarty and Habets}{2018}]{Chakrabarty2018}
S.~Chakrabarty and E.~A.~P. Habets, ``A {Bayesian} approach to informed spatial
  filtering with robustness against {{DOA}} estimation errors,''
  \emph{{IEEE/ACM} Trans. Audio, Speech, Lang. Process.}, vol.~26, no.~1, pp.
  145--160, Jan. 2018.
  
\bibitem[\protect\astroncite{Cox \textit{et al.}}{1987}]{Cox1987}
H.~Cox, R.~M. Zeskind, and M.~M. Owen, ``Robust adaptive beamforming,''
  \emph{{IEEE} Trans. Acoust., Speech, Signal Process.}, vol.~35, no.~10, pp.
  1365--1376, Oct. 1987.

\bibitem[\protect\astroncite{Eaton \textit{et al.}}{1987}]{Eaton2015}
J.~Eaton, N.D.~Gaubitch, A.H~Moore, and P.A.~Naylor, ``The ACE challenge—Corpus description and performance evaluation", \emph{2015 IEEE Workshop on Applications of Signal Processing to Audio and Acoustics (WASPAA)}, Oct. 2015, pp. 1--5.

\bibitem[\protect\astroncite{Ehrenberg \textit{et al.}}{2010}]{Ehrenberg2010}
L.~Ehrenberg, S.~Gannot, A.~Leshem, and E.~Zehavi, ``Sensitivity analysis of
  {{MVDR}} and {{MPDR}} beamformers,'' in \emph{{IEEE} Conv. Electrical and
  Electronics Engineers in Israel}, Nov. 2010, pp. 416--420.

\bibitem[\protect\astroncite{Gannot \textit{et al.}}{2001}]{Gannot2001}
S.~Gannot, D.~Burshtein, and E.~Weinstein, ``Signal enhancement using
  beamforming and nonstationarity with applications to speech,'' \emph{{IEEE}
  Trans. Signal Process.}, vol.~49, no.~8, pp. 1614--1626, Aug. 2001.

\bibitem[\protect\astroncite{Garofolo \textit{et al.}}{1993}]{Garofolo1993a}
J.~S. Garofolo, L.~F. Lamel, W.~M Fisher, J.~G. Fiscus, D.~S. Pallett and N.~L. Dahlgren, ``DARPA Timit Acoustic-Phonetic Continuous Speech Corpus,'' Linguistic Data Consortium (LDC), Philadelphia, 1993.

\bibitem[\protect\astroncite{Hu \textit{et al.}}{2008}]{Hu2008}
Y.~Hu and P.~C.~Loizou, ``Evaluation of Objective Quality Measures for Speech Enhancement,'' in IEEE Transactions on Audio, Speech, and Language Processing, vol. 16, no. 1, pp. 229-238, Jan. 2008.


\bibitem[\protect\astroncite{ITU-T}{1993}]{ITU_T_P56}
ITU-T. ``Objective measurement of active speech level,'' Intl. Telecommunications
  Union ({ITU-T}), Recommendation P.56, Mar. 1993.
 
\bibitem[\protect\astroncite{ITU-T}{2003}]{ITU_T_P862}
ITU-T. ``Perceptual evaluation of speech quality ({{PESQ}}), an objective method for
  end-to-end speech quality assessment of narrowband telephone networks and
  speech codecs,'' Intl. Telecommunications Union ({ITU-T}), Recommendation
  P.862, Nov. 2003. 
  
\bibitem[\protect\astroncite{Jarret \textit{et al.}}{2017}]{Jarrett2017}
D.~P. Jarrett, E.~A.~P. Habets, and P.~A. Naylor, \emph{Theory and Applications
  of Spherical Microphone Array Processing}, ser. Springer Topics in Signal
  Processing.\hskip 1em plus 0.5em minus 0.4em\relax Springer International
  Publishing, 2017.

\bibitem[\protect\astroncite{Kayser \textit{et al.}}{2009}]{Kayser2009}
H. Kayser, S.~D. Ewert, J. Anem\"{u}ller, T. Rohdenburg, V. Hohmann, and B. Kollmeier, ``Database of Multichannel In-ear and Behind-the-ear Head-related and Binaural Room Impulse Responses'', \emph{EURASIP J. Adv. Signal Process}, Hindawi Publishing Corp, New York, NY, United States, vol.~2009, no.~6, pp.~6:1--6:10, 2009.

\bibitem[\protect\astroncite{Klasen \textit{et al.}}{2007}]{Klasen2007a}
T.~J. Klasen, T.~V. den Bogaert, M.~Moonen, and J.~Wouters, ``Binaural noise
  reduction algorithms for hearing aids that preserve interaural time delay
  cues,'' \emph{{IEEE} Trans. Signal Process.}, vol.~55, no.~4, pp. 1579--1585,
  Apr. 2007.

\bibitem[\protect\astroncite{Li \textit{et al.}}{2003}]{Li2003}
J.~Li, P.~Stoica, and Z.~Wang, ``On robust {Capon} beamforming and diagonal
  loading,'' \emph{{IEEE} Trans. Signal Process.}, vol.~51, no.~7, pp.
  1702--1715, 2003.
  
\bibitem[\protect\astroncite{Lollmann \textit{et al.}}{2017}]{Lollmann2017}
H.~W. L\"ollmann, A.~H. Moore, P.~A. Naylor, B.~Rafaely, R.~Horaud, A.~Mazel,
  and W.~Kellermann, ``Microphone array signal processing for robot audition,''
  in \emph{Proc. Joint Workshop on Hands-free Speech Communication and
  Microphone Arrays ({HSCMA})}, Mar. 2017, pp. 51--55.

\bibitem[\protect\astroncite{Markovich \textit{et al.}}{2009}]{Markovich2009}
S.~Markovich, S.~Gannot, and I.~Cohen, ``Multichannel eigenspace beamforming in
  a reverberant noisy environment with multiple interfering speech signals,''
  \emph{{IEEE} Trans. Audio, Speech, Lang. Process.}, vol.~17, no.~6, pp.
  1071--1086, Aug. 2009.

\bibitem[\protect\astroncite{Markovich-Golan and Gannot}{2015}]{Markovich-Golan2015}
S.~{Markovich-Golan} and S.~Gannot, ``Performance analysis of the covariance
  subtraction method for relative transfer function estimation and comparison
  to the covariance whitening method,'' in \emph{Proc. {IEEE} Intl. Conf. on
  Acoustics, Speech and Signal Processing ({ICASSP})}, Apr. 2015, pp. 544--548.

\bibitem[\protect\astroncite{Moore \textit{et al.}}{2018}]{Moore2018a}
A.~H. Moore, L.~Lightburn, W.~Xue, P.~A. Naylor, and M.~Brookes, ``Binaural
  mask-informed speech enhancement for hearing aids with head tracking,'' in
  \emph{Proc. Intl. Workshop on Acoustic Signal Enhancement ({IWAENC})}, Tokyo,
  Japan, Sept. 2018.

\bibitem[\protect\astroncite{Moore \textit{et al.}}{2019}]{Moore2019}
A.~H. Moore, W.~Xue, P.~A. Naylor, and M.~Brookes, ``Noise covariance matrix
  estimation for rotating microphone arrays,'' \emph{{IEEE/ACM} Trans. Audio,
  Speech, Lang. Process.}, vol.~27, no.~3, pp. 519--530, Mar. 2019.

\bibitem[\protect\astroncite{Moore \textit{et al.}}{2019b}]{Moore2019b}
A.~H. Moore, J.~M. de~Haan, M.~S. Pedersen, P.~A. Naylor, M.~Brookes, and
  J.~Jensen, ``Personalized signal-independent beamforming for binaural hearing
  aids,'' \emph{J. Acoust. Soc. Am.}, vol.~145, pp.2971-–2981. 2019.


\bibitem[\protect\astroncite{Moore \textit{et al.}}{2020}]{Moore2020}
A.~H. Moore, R.~R. Vos, P.~A. Naylor, and M.~Brookes, ``Evaluation of the performance of a model-based adaptive beamformer,'' \emph{in Proc Speech in Noise Workshop}, Toulouse, France, Jan. 2020.

\bibitem[\protect\astroncite{Naylor \textit{et al.}}{2019}]{Moore2019a}
A.~H. Moore, P.~A. Naylor, and M. Brookes, ``Improving robustness of adaptive beamforming for hearing devices,'' \emph{in Proc Intl Symp on Auditory and Audiological Research}, Nyborg, Denmark, Aug. 2019.


\bibitem[\protect\astroncite{Rafaely}{2015}]{Rafaely2015}
B.~Rafaely, \emph{Fundamentals of Spherical Array Processing}, ser. Springer
  Topics in Signal Processing. Berlin
  Heidelberg: Spring{\-}er-Ver{\-}lag, 2015.

\bibitem[\protect\astroncite{Schwartz \textit{et al.}}{2016}]{Schwartz2016}
O.~Schwartz, S.~Gannot, and E.~A.~P. Habets, ``Joint estimation of late
  reverberant and speech power spectral densities in noisy environments using
  frobenius norm,'' in \emph{Proc. European Signal Processing Conf. (EUSIPCO)},
  Aug. 2016, pp. 1123--1127.
	
\bibitem[\protect\astroncite{Schwarz \textit{et al.}}{2015}]{Schwarz2015}
A.~Schwarz, and W.~Kellermann, ``Coherent-to-diffuse power ratio
  estimation for dereverberation,'' \emph{{IEEE/ACM} Trans. Audio,
   Speech, Lang. Process.}, vol.~23, no.~6, pp. 1006--1018, Jun. 2015.	

\bibitem[\protect\astroncite{Taal \textit{et al.}}{2011}]{Taal2011}
C.~H. Taal, R.~C. Hendriks, R.~Heusdens, and J.~Jensen, ``An algorithm for
  intelligibility prediction of time-frequency weighted noisy speech,''
  \emph{{IEEE} Trans. Audio, Speech, Lang. Process.}, vol.~19, no.~7, pp.
  2125--2136, Sept. 2011.
  
\bibitem[\protect\astroncite{Tamai \textit{et al.}}{2004}]{Tamai2004}
Y.~Tamai, S.~Kagami, Y.~Amemiya, Y.~Sasaki, H.~Mizoguchi, and T.~Takano,
  ``Circular microphone array for robot's audition,'' in \emph{Sensors, 2004.
  {{Proceedings}} of {{IEEE}}}, Oct. 2004, pp. 565--570, vol.2.

\bibitem[\protect\astroncite{Thiergart and Habets}{2003}]{Thiergart2013}
O.~Thiergart and E.~A.~P. Habets, ``An informed {{LCMV}} filter based on
  multiple instantaneous direction-of-arrival estimates,'' in \emph{Proc.
  {IEEE} Intl. Conf. on Acoustics, Speech and Signal Processing ({ICASSP})},
  May 2013, pp. 659--663.
  
\bibitem[\protect\astroncite{van Trees}{2002}]{Trees2002a}
H.~L. {van Trees}, \emph{Optimum Array Processing}, ser. Detection, Estimation
  and Modulation Theory.\hskip 1em plus 0.5em minus 0.4em\relax John Wiley \&
  Sons, Inc., 2002.
  
\bibitem[\protect\astroncite{Yilmaz and Rickard}{2004}]{Yilmaz2004}
O.~Yilmaz and S.~Rickard, ``Blind separation of speech mixtures via
  time-frequency masking,'' \emph{{IEEE} Trans. Signal Process.}, vol.~52,
  no.~7, pp. 1830--1847, July 2004.
  

==> biographies_IEEE_submission_compatible_13pages.tex <==
%\vskip -2\baselineskip plus -1fil
%\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_sina}}]{Sina Hafezi}
is a post-doctoral Research Associate at Imperial College London. He received the BEng degree in Electronic Engineering in 2012 and the MSc degree in Digital Signal Processing in 2013 both from Queen Mary, University of London, UK. He worked in the Centre for Digital Music as a researcher and software engineer on autonomous multitrack mixing systems. In 2018, he received his PhD in acoustic source localisation using spherical microphone arrays at Imperial College London, UK. He spent 2.5 years at Silixa as Senior Signal Processing Engineer developing algorithms and software. In 2021, he re-joined Imperial College London, where he has contributed to academic and industrial projects on hearing aids and spatial audio. His research interests are microphone array processing, spatial audio, denoising, source localisation and room acoustic modelling with applications for augmented and virtual reality. In 2023, he founded Circumix, an XR audio technology startup.
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_alastair}}]{Alastair H. Moore}
(M'13) is  a  Research Fellow at  Imperial  College  London  and  spatial  audio  consultant  with  Square  Set  Sound.  He  received  the M.Eng. degree in Electronic Engineering with Music Technology Systems in 2005 and the Ph.D. degree in 2010, both from the University of York, York, U.K. He  spent  3  years  as  a  Hardware  Design  Engineer for Imagination Technologies PLC designing digital radios  and  networked  audio  consumer  electronics products. In 2012, he joined Imperial College, where he has contributed to a series of projects in the field of speech and audio processing applied to voice over IP, robot audition, and hearing  aids.  Particular  topics  of  interest  include  microphone  array  signal processing, modeling and characterization of room acoustics, dereverberation, and  spatial  audio  perception.
\end{IEEEbiography}


%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_pierre.jpg}}]{Pierre H. Guiraud} 
is a post-doctoral Research Associate at Imperial College
London. After enrolling in a double degree program, he received a MSc in Engineering from the Ecole Centrale de Lille, France, as well as a Master in Engineer Acoustic from the Technical University of Denmark in Copenhagen in 2017. He went on to pursue a PhD at the IEMN in Lille, France, about the thermoacoustic sound generation in porous metamaterials. He obtained his PhD in 2020 and joined Imperial College London in 2021 working on several projects including the SPEAR Challenge, ELO-SPHERES and spatial audio perception in a virtual reality environment.
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_naylor}}]{Patrick A. Naylor}
(M’89, SM’07, F’20) is Professor of Speech and Acoustic Signal Processing at Imperial  College  London.  He  received  the  BEng  degree in  Electronic  and  Electrical  Engineering  from  the University  of  Sheffield,  UK,  and  the  PhD  degree from  Imperial  College  London,  UK.  His  research interests are in speech, audio and acoustic signal processing. His current research addresses microphone array   signal   processing,   speaker   diarization,   and multichannel speech enhancement for application to binaural  hearing  aids  and  robot  audition. In addition to his academic research, he enjoys several collaborative links with industry. He is currently a member of the Board of Governors of the IEEE Signal Processing Society and President of  the  European  Association  for  Signal  Processing  (EURASIP).  He  was formerly Chair of the IEEE Signal Processing Society Technical Committee on Audio and Acoustic Signal Processing. He has served as an associate editor of  IEEE  Signal  Processing  Letters  and  is  currently  a  Senior  Area  Editor  of IEEE Transactions on Audio Speech and Language Processing.
\end{IEEEbiography}

%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_jacob.png}}]{Jacob Donley}
is a research scientist at Meta Reality Labs Research in Redmond, WA with previous experience lecturing in Signals and Systems at the University of Wollongong (UOW) and Engineering at Western Sydney University. He holds a Bachelor of Engineering Honours (Computer) (UOW), a Ph.D. (UOW) with research focused on Digital Signal Processing (DSP) aimed at improving the reproduction of personal sound in shared environments, and a graduate certificate in Artificial Intelligence (AI) from Stanford University. Jacob’s research interests are in signal processing, speech enhancement, machine learning, array processing (microphone and loudspeaker), beamforming, and multi-zone sound field reproduction. Jacob has received awards and scholarships from Telstra Corporation Limited, the Australian Department of Education and Training, and the University of Wollongong.


\end{IEEEbiography}


%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_vladi.png}}]{Vladimir Tourbabin}
(M’16) is a Research Science Manager at Meta. He received the B.Sc. degree (summa cum laude) in materials science
and engineering in 2005, the M.Sc. degree (cum laude) in electrical and computer engineering in 2011, and the PhD degree in electrical and computer engineering in 2016. All three degrees are from Ben-Gurion University of the Negev, Israel. After the graduation, he has joined the General Motors’ Advanced Technical Center in Israel, to work on microphone array processing solutions for speech recognition. Since 2017, Dr. Tourbabin is with Reality Labs Research @ Meta working on research and advanced development of audio signal processing technologies for augmented and virtual reality applications.
\end{IEEEbiography}


%\vskip -2\baselineskip plus -1fil
\vskip 0pt plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{graphics/author_thomas.png}}]{Thomas Lunner's}
career has focused on man-machine issues related to the correlation between hearing and cognition. He was the first scientist to convincingly show the importance of cognitive ability in relation to being able to recognize speech in adverse listening conditions. He also demonstrated how working memory was a significant factor for the selection of optimum signal processing in hearing aids to be fitted to a particular individual. These studies led to increasing cooperation with other research groups globally, and the establishment of cognitive hearing science as a research field of its own. Dr. Lunner’s Ph.D. research in the mid-1990s resulted in patented signal processing algorithms which led to the development of the first digital hearing aid manufactured by Oticon. The core of this project was a digital filter bank which provided the necessary tuning flexibility with an equally important low power consumption. The filter bank was used in several successive hearing aid models in the years that followed, fitted to millions of hearing aid users worldwide. Two of the models were awarded the European Union’s prestigious technology prize, the IST Grand Prize in 1996 and in 2003. Currently, he leads research in Superhuman Hearing at Meta Reality Labs Research.
\end{IEEEbiography}





%\vskip -2\baselineskip plus -1fil
%\vskip 0pt plus -1fil

==> block_diagram.tex <==
% figure 1
% \begin{figure}
% \centering
\begin{tikzpicture}[node distance=2cm]
% first the nodes:
% \node(HRTFconv) [vprocess3] {text};
% \node(in_mid) [input, left of=HRTFconv, node distance=3cm] {};
\small
\node(in_mid) [input]{};
\node(in1) [input, above of=in_mid, node distance = 1.5*\bigyshift] {};
\node(in2) [input, above of=in_mid, node distance = 0.5*\bigyshift] {};
\node(in3) [input, above of=in_mid, node distance = -0.5*\bigyshift] {};
\node(in4) [input, above of=in_mid, node distance = -1.5*\bigyshift] {};
\node(HRTFconv) [vprocess3, right of=in2, node distance=2.5cm] { 
\parbox{\widthof{microphone}}{\centering
    $*$ HRTF \\
    and \\
    microphone \\
    response}};
\node(norm) [vprocess4, right of=in_mid, node distance=5.0cm] {\parbox{\widthof{ microphone}}{\centering
    normalise levels to \SI{0}{\dB} at reference microphone}};
\node(ampl) [hprocess, above of=norm, xshift=1.0cm, node distance=2.5cm] {\parbox{\widthof{levels ($\ampTarget, \ampInterferer, \ampBabble, \ampSensornoise$)}}{\centering
    desired relative levels $\ampTarget, \ampInterferer, \ampBabble, \ampSensornoise$}};
\node(mult_mid) [point, right of=norm, node distance=2.0cm]{};
\node(multpoint1) [operator, above of=mult_mid, node distance=1.5*\bigyshift]{$\times$};
\node(multpoint2) [operator, above of=mult_mid, node distance=0.5*\bigyshift]{$\times$};
\node(multpoint3) [operator, above of=mult_mid, node distance=-0.5*\bigyshift]{$\times$};
\node(multpoint4) [operator, above of=mult_mid, node distance=-1.5*\bigyshift]{$\times$};
\node(addpoint) [operator, right of=mult_mid, node distance=1cm]{$+$};
\node(outpoint) [point, right of=addpoint, node distance=1.5cm]{};

% then the connections:
\draw[arrow] (in1) -- node[anchor=south]{$\sigTarget$}(in1-| HRTFconv.west);
\draw[arrow] (in2) -- node[anchor=south]{$\sigInterferer$}(in2-| HRTFconv.west);
\draw[arrow] (in3) -- node[anchor=south]{$\sigBabble$}(in3-| HRTFconv.west);
\draw[line] (in4) -- node[anchor=south]{$\sigSensornoise$}(in4-| HRTFconv.west);
\draw[arrow] (in1-| HRTFconv.east) -- (in1-| norm.west);
\draw[arrow] (in2-| HRTFconv.east) -- (in2-| norm.west);
\draw[arrow] (in3-| HRTFconv.east) -- (in3-| norm.west);
\draw[arrow] (in4-| HRTFconv.west) -- (in4-| norm.west);
\draw[arrow] (in1-|norm.east) -- (multpoint1);
\draw[arrow] (in2-|norm.east) -- (multpoint2);
\draw[arrow] (in3-|norm.east) -- (multpoint3);
\draw[arrow] (in4-|norm.east) -- (multpoint4);
\draw[arrow] (ampl.south) -- (multpoint1);
\draw[arrow] (ampl.south) -- (multpoint2);
\draw[arrow] (ampl.south) -- (multpoint3);
\draw[arrow] (ampl.south) -- (multpoint4);
\draw[arrow] (multpoint1) -- (addpoint);
\draw[arrow] (multpoint2) -- (addpoint);
\draw[arrow] (multpoint3) -- (addpoint);
\draw[arrow] (multpoint4) -- (addpoint);
\draw[arrow] (addpoint) -- node[anchor=south]{$\sigMixed$}(outpoint);
% then the dotted lines
% and dashed
\end{tikzpicture}
% \end{figure}

==> figuredefs.tex <==

\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{line} = [thick]


\def\bigyshift{1cm}

\def\myyshift{0.2cm}
\def\myyshiftb{0.15cm} % use this one for the distance from the dotted lines to the boxes
\def\myxshift{0.2cm}


\tikzstyle{vprocess3} = [rectangle, minimum width=1cm, minimum height=2.5*\bigyshift, text centered, draw=black]
\tikzstyle{vprocess4} = [rectangle, minimum width=1cm, minimum height=3.5*\bigyshift, text centered, draw=black]

\tikzstyle{hprocess} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
% \tikzstyle{hprocesssmall} = [rectangle, minimum width=1.5cm, minimum height=0.6cm, text centered, draw=black]
% \tikzstyle{hprocesssmall2} = [rectangle, minimum width=0.75cm, minimum height=0.6cm, text centered, draw=black]
% \tikzstyle{vprocess} = [rectangle, minimum width=1cm, minimum height=3cm, text centered, draw=black]
% \tikzstyle{vprocesssmall} = [rectangle, minimum width=1cm, minimum height=2.5cm, text centered, draw=black]
\tikzstyle{operator} = [circle, minimum width=0.4cm,inner sep=0cm, text centered, draw=black, fill opacity = 1]

\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{point} = [coordinate]


==> glossary.tex <==
% \usepackage[colorlinks]{hyperref}
% \usepackage[symbols,nogroupskip,sort=none]{glossaries-extra}
List of symbols used:

\begin{description}
\item[$\rtfArrayFreqVec$] array steering vector
\item[$\filtFreqSteeringVec$] steering vector
\item[$\covBasisMat$] matrix containing the basis vectorized covariance matrices
\item[$\direct$] direct
\item[$\filtArrayTime$] acoustic impulse response
\item[$\filtArrayFreqVec$] array response?
\item[$\eye$] the identity matrix
\item[$\idPW$] plane component index
\item[$\numPW$] number of plane components
\item[$\idPWincl$] plane wave index in the compact model
\item[$\numPWincl$] number of plane waves in the compact model
\item[$\idSource$] source index
\item[$\stftFrame$] frame index (STFT domain)
\item[$\numSource$] number of sources
\item[$\idMic$] microphone index
\item[$\numMic$] number of microphones
\item[$\reflected$] reflected [not used now I think]
\item[$\covMatFreqVec$] real-vectorized covariance matrix
\item[$\covMatFreq$] covariance matrix used to calculate beamformer weights
\item[$\covUnitPlanewave$] covariance of the plane wave noise component
\item[$\covRobust$] robust noise covariance 
\item[$\covUnitDiffuse$] covariance of the diffuse noise component
\item[$\covUnitWhite$] covariance of the sensor noise component
\item[$\covMic$] sample covariance matrix
\item[$\covMicModel$] estimated covariance matrix
\item[$\covMicSmoothEst$] estimated sample covariance matrix
\item[$\sigSourceTime$] emitted signal (time domain)
\item[$\sigSourceFreq$] emitted signal (STFT domain)
\item[$\sigSourceModFreq$] signal due to the dominant source at the reference microphone (STFT domain)
\item[$\idTime$] time index (time domain)
\item[$\sigMicWhiteTime$] sensor noise (time domain)
\item[$\sigMicWhiteFreq$] sensor noise (STFT domain)
\item[$\sigMicWhiteFreqVec$] sensor noise signal 
\item[$\filtBfFreqVec$] beamformer weights (frequency domain)
\item[$\sigMicSourceTime$] source signal (time domain)
\item[$\sigMicSourceFreq$] source signal (STFT domain)
\item[$\sigMicTime$] received signal (time domain)
\item[$\sigMicFreq$] received signal (STFT domain)
\item[$\sigMicFreqVec$] received signal (STFT domain)
\item[$\sigMicModFreqVec$] estimated microphone signal?
\item[$\alpha$] smoothing time constant
\item[$\sigMicDiffuseFreqVec$] diffuse noise signal (vector) (freq domain) 
\item[$\sigMicDiffuseFreq$] diffuse noise signal (freq domain) 
\item[$\scalarLoading$] diagonal loading factor for $\covRobust$
\item[$\covCondNumLimit$] maximum permitted condition number of $\covRobust$
\item[$\covEigenvalue$] eigenvalue of covariance matrix
\item[$\LagMultOptVec$] vector of Lagrange multipliers
\item[$\stftFreq$] frequency index (STFT domain)
\item[$\pi$] pi
\item[$\powSourceModFreq$] power(s) of the plane-wave noise component(s)
\item[$\powDiffuse$] power of the diffuse noise component
\item[$\powWhite$] power of the sensor noise component
\item[$\powOptVec$] vector of component powers
\item[$\doa$] direction of arrival \ac{DOA} of the plane-wave component(s)
\item[$\az$] azimuth angle
\end{description}
%
%
\medskip
List of mathematical operators
\begin{description}
\item[$\mathbf{\dot{(\cdot)}}$] an estimated quantity
\item[$\expectOp\{\cdot\}$] expectation
\item[$(\cdot)^{\hermitianOp}$] conjugate transpose
\item[$\sum$] sum
\item[$||\cdot||_{F}$] the Frobenius norm
\item[$\int$] integral
\item[$\invMacro{(\cdot)}$] inverse
\item[$\argmin$] minimisation operator
\item[$\forall$] for all
\end{description}

==> references-bibfile.tex <==
\bibliographystyle{bibtex/bib/IEEEtran}
%\bibliographystyle{IEEEtranN}
\bibliography{bibtex/bib/sapstrings,bibtex/bib/sapref,bibtex/bib/extras}https://www.overleaf.com/project/5e452f51b0b0ea000107a402
